Economic Analyses of Security Investments on Cryptocurrency Exchanges

Cryptocurrency exchanges are frequently targeted and compromised by cyber-attacks, which may lead to significant losses for the depositors and closure of the affected exchanges. These risks threaten the viability of the entire public blockchain ecosystem since exchanges serve as major gateways for participation in public blockchain technologies. In this paper, we develop an economic model to capture the short-term incentives of cryptocurrency exchanges with respect to making security investments and establishing transaction fees. Using the model, we derive conclusions regarding an exchange's optimal economic decisions, and illustrate key features of these conclusions using graphs based on real-world data. Our security investment model exhibits horizontal scaling properties with respect to reducing exposure to losses, and may be of special interest to exchanges operating in markets with high price volatility.

==> ideas.tex <==
\section{Ideas}

\subsection{Aron's Initial Thoughts (October 4th, 2015)}

\paragraph{Players} \ \\

Users:
\begin{itemize}
\item A Bitcoin user's primary strategic decision (with regard to exchanges) is choosing which exchange(s) to use. To make this decision, a user should take into account both the fee and the risk of losing money (note that risk comes both from fraudulent exchanges and from benign exchanges suffering security incidents). Since most users are risk-averse in practice (at least in this respect), they will not simply pick the exchange that maximizes their expected gain, but rather diversify by choosing a set of multiple exchanges. As usual, this risk-aversion can be modeled using utility functions, and we can easily compute the utility maximizing set assuming that exchanges fail independently of each other.
\item It is important to note that users do not have to store bitcoins (or any other currency) at exchanges permanently, since they can withdraw from their accounts as soon as the currency is exchanged. Moreover, they can further reduce risks by not exchanging large amounts at once, but rather exchanging smaller amounts multiple times. The reason why users risk their money is comfort: exchanging larger amounts at once and leaving money in the exchange's account until needed is convenient. Hence, there is a trade-off between convenience (i.e., saving time and effort) and security. We can study this trade-off by allowing users to choose the amount of money to be risked, and formulating a user's utility as a function of both the successfully exchanged (i.e., not lost) and the un-exchanged money (the latter obviously being less useful). 
\end{itemize}

Exchanges:
\begin{itemize}
\item A Bitcoin exchange has a lot of strategic decisions to make. First, they have to select a fee, taking into account that a higher fee might lead to a smaller market share (however, it might also lead to a higher market share, see below).
\item Second, they can choose how much to invest in security. Data shows that a lot of exchanges have suffered breaches, which lead to considerable financial and reputation losses, so investing in security to reduce the risk incidents is important for exchanges. Unfortunately, there is an information asymmetry between the users and the exchanges, since the former do not know how much the latter have invested, and hence, how risky they are. This might lead to underinvestment, unless the exchanges can somehow signal their true risk levels to the users.
\item Third, exchanges may also decide to become malicious and steal the users' money. This decision should be based (at least in part) on whether the amount of money currently stored at the exchange exceeds the present value of all future profits made from the exchange. Hence, a higher fee might signal to the users that the exchange is less risky (and lead to a higher market share), since the exchange has no incentives to become malicious if it is very profitable. Alternatively, we can model exchanges as inherently malicious and benign (see Bayesian games below).
\item Finally, an exchange might try to build reputation or signal its risk level to the users in some other way (e.g., the ESORICS paper).
\end{itemize}

Attackers: Instead of simply assuming that the risk of security incidents is somehow determined by the security investment levels, we could assume strategic attackers, who pick their targets taking into account both the security levels and the amounts of money stored at the exchanges.

\paragraph{Game-theoretic tools}

\begin{itemize}
\item Mean-field game theory: Since the number of users is very large, we could assume that they are uniform, and model them as a single decision maker.
\item Bayesian game: We could assume that exchanges are inherently malicious or benign (obviously leading to different payoff functions and strategy sets), but users only know the probability of an exchange being malicious (or benign). If we want to combine the model with data, this probability could be estimated for a given exchange from certain factors using Tyler's paper.
\item Signaling game: The above Bayesian game is a prime candidate for modeling it as a signaling game, with the exchange being the send and the users being the receivers.
\end{itemize}

\paragraph{Research questions}

\begin{itemize}
\item What is the best strategy for the users? How should they diversify to minimize risk and maximize utility?
\item What is the best strategy for benign exchanges? How should they signal their risk level or their benign nature?
\item How does the equilibrium of the players' strategies compare to the social optimum (i.e., what is the price of anarchy / stability)?
\item Do the players' best responses lead to a monopoly (which may result in system(at)ic risk)?
\end{itemize}


\subsection{Discussion (October 5th, 2015)}

What Tyler did?
\begin{itemize}
\item	With Nicolas and Janos Szurdi: collect data on exchanges since Spring 2013
\item	Collected additional information: 4 boolean variables → security signaling (bragging; cold storage for wallets; two others)
\begin{itemize}
\item	Security measures could make things safer or could signal to users (and thereby contribute to success) and prospective attackers (displacement effect)
\item	2-factor authentication
\item	Bug bounty program
\item	Security audit; penetration test
\item	Cold storage (does this slow down the exchange? Or unambiguously better?)
\item	Can users verify any of those?
\end{itemize}
\item	Whether there is an influence on getting breached or closed: only influence was 2-factor authentication (negatively correlated with attack, and closure)
\item	Know nothing about users’ perceptions regarding security measures
\item	Transaction volume at the exchange is correlated with experiencing a breach; also associated with longer lifetime
\item	Public report on a breach → no relationship with lifetime of exchange
\end{itemize}

\noindent Other thoughts:
\begin{itemize}
\item	Data on security posture of different exchanges could be available
\item	Could explain security measures and signals and show evidence that they exist?
\item	What are motivations for attacks on exchanges? There are DDoS, but that’s pretty close to previous papers. Theft of bitcoins: exchanges are like any other bank.
\item	What about liability? Are they insured? → but might be forced to reimburse; present value and future profit.
\item	An attack arrives (whether internal or external) → then exchange can reimburse, fold, or just keep on going.  → what are the strategies for the users?
\item	Why not simply spread risk around?
\item	Delay on getting money in and out… → users may want to do some trading on the platform → rational and bounded rational reasons (users are lethargic)
\item	Can we find out what people are actually doing? By reading entries on blogs.
\item	DDoS might be like creating your own insider information → Slow down trading to get in front of trading… → keep as future work thought
\item	Should the exchanges be fraudulent
\item	First 2013 study: whether more risky exchange offer better exchange rates → but there could be also a market failure → bad exchanges could mimic good exchanges
\begin{itemize}
\item	Markets control the fees
\item	Not modeling exchange rates
\item	One factor that helps to attract more users is low bid-ask spread rather than being on a thin market → additional fee that kinds of depends on size → liquidity aspects (how quickly can you get out)
\item	But our focus is on understanding trustworthiness
\end{itemize}
\item	Tyler can take a look at history: why where there significant rises and falls of exchanges
\end{itemize}



